Stripped and Enriched: The Role of Ram-Pressure in Shaping Chemical Enrichment of Galaxies at Intermediate Redshift

The chemical evolution of galaxies is shaped by their star formation histories and the exchange of gas with their environments. Metallicity provides key insights into these processes, reflecting the interplay between star formation and gas flows. A fundamental aspect of this evolution is the mass-metallicity relation, which captures the strong correlation between a galaxy stellar mass ($M_\star$) and its gas-phase oxygen abundance. In this study, we use MUSE observations to analyze star-forming disc galaxies in 12 clusters within the redshift range $0.3 < z < 0.5$. Galaxies were classified into three groups: ram-pressure stripping (RPS), control cluster, and control field. For the first time, we investigate the impact of RPS on gas-phase metallicities across a wide mass range of galaxies at intermediate redshift, comparing RPS galaxies to counterparts in both cluster and field environments. By analyzing the integrated flux within galactic disks, our results reveal that, on average, RPS induces a metallicity enhancement of 0.2 dex over non-stripped galaxies. Contrary to the prevailing view that cluster membership alone drives metallicity enrichment, we find that control cluster galaxies exhibit metallicities comparable to field galaxies at a given $M_\star$, with only RPS galaxies displaying significantly higher metal content, highlighting the unique role of RPS in shaping the chemical properties of galaxies. These differences become more pronounced at lower $M_\star$, indicating that environmental influences play a more critical role in shaping the chemical evolution of lower-mass galaxies. Our findings suggest that both enhanced star formation rates and suppressed gas inflows -- consequences of ram pressure stripping -- drive the elevated metallicity observed in RPS galaxies.

==> tempo.tex <==

whole sample:

RPS 28, 12 no ha 

     3 not a member , 1 interacting , 1 contaminated , 1 <60\% spxs , 1 PSB

CC 40, 12 no Ha

   3 AGN/Outflow  , 2 interacting , 1 not a member, 12 low snr/no gas 
    
CF 12, 4 no ha
    1 possible!AGN , 2 contamination , 1 low snr/no gas

metallicity:
21 RPS, 6 no ha  (put a box)
22 CC, 6 no ha
9 CF, 2 no ha

SNR>2
60\% usable spaxels
have Ha+NII or OII



CC = [

'A370_10', 'A370_15', 'A370_18', 'A370_23', 'AS1063NE_05',
        'AS1063NE_08', 'AS1063SW_03', 'AS1063SW_04', 'MACS0940_04',
        'MACS0940_05',  'MACS1206_05', 'MACS1206_15',
        'MACS1206_17', 'SMACS2031_03' , 'MACS1206_02', 'MACS1206_12', 'RXJ1347_01', 'RXJ1347_04',
        'SMACS2131_04', 'SMACS2131_07’]

_______________



3 AGN/Outflow  ,
MACS1206_15,
A2744_17,
A2744_18

 
2 interacting , 
A2744_23
A2744_14




1 not a member, 
MACS0940_07

12 low snr/no gas

A370_13
A370_11
A2744_21
A370_12
MACS1206_14
A2744_11
A2744_12
A2744_13
A2744_15
A2744_19
A2744_22
A370_19

#####
#####
#####


RPS = 

'A2744_03', 'A2744_04', 'A2744_06', 'A2744_09', 'A2744_10',
        'A2744_16', 'A370_01', 'A370_03', 'A370_06', 'A370_07', 'A370_08',
'A370_09', 'A370_17', 'MACS0416N_01', 'SMACS2031_01’, 'MACS1206_01', 'MACS1206_03', 'MACS1206_07', 'MACS1206_10',
        'SMACS2131_01', 'SMACS2131_03'

____________

A2744_14 (superposition)
MACS0940_01 (contaminated)
MACS0416S_02 (contamination)
MACS0940_03
(less than 60%)
MACS1206_08
 (No mem)
MACS1206_21 
 (no Mem)
MACS1206_22
 (No Memb)


3 not a member ,
1 interacting , 
1 contaminated , 
1 <60\% spxs ,
1 PSB

